On the impact of semantic transparency on understanding and reviewing social goal models

Context: i* is one of the most influential languages in the Requirements Engineering research community. Perhaps due to its complexity and low adoption in industry, it became a natural candidate for studies aiming at improving its concrete syntax and the stakeholders' ability to correctly interpret i* models. Objectives: We evaluate the impact of semantic transparency on understanding and reviewing i* models, in the presence of a language key. Methods: We performed a quasi-experiment comparing the standard i* concrete syntax with an alternative that has an increased semantic transparency. We asked 57 novice participants to perform understanding and reviewing tasks on i* models, and measured their accuracy, speed and ease, using metrics of task success, time and effort, collected with eye-tracking and participants' feedback. Results: We found no evidence of improved accuracy or speed attributable to the alternative concrete syntax. Although participants' perceived ease was similar, they devoted significantly less visual effort to the model and the provided language key, when using the alternative concrete syntax. Conclusions: The context provided by the model and language key may mitigate the i* symbol recognition deficit reported in previous works. However, the alternative concrete syntax required a significantly lower visual effort.

==> 2_background.tex <==
%----------------------------------------------------------------------------------------------
%----------------------------------------------------------------------------------------------
% JÁ NÃO SE ESTÁ A USAR ESTA SECÇÃO

\section{Background}
\label{sec:background}

\subsection{\textit{i*} framework}
The \textit{i*} \cite{Yu1995} framework was designed for modelling and analysis of organizational environments and their information systems.
%Its focus is on the concept of intentional actor. %In their organizational environment 
An \textit{Intentional actor} is a central concept of the approach. 
Actors are viewed as having intentional properties such as \textit{goals}, \textit{beliefs}, \textit{abilities} and \textit{commitments}. i* has two main models: the Strategic Dependency (SD) model and the Strategic Rationale (SR) model. The SD model describes the dependency relationships among the actors in an organizational context. Here, an actor (called \textit{depender}) depends on another actor (called \textit{dependee}) to achieve goals and softgoals, to perform tasks and to obtain resources. The SR model %adds %a 
%more details than the SD model, since it 
focuses on %the 
modelling %of 
intentional elements and relationships internal to actors. Intentional elements (goals, softgoals, tasks and resources) are related by means-end or decomposition links. Means-end links are used to link goals (ends) to tasks (means) %in order 
to specify alternative ways to achieve goals. Decomposition links are used to decompose tasks. %A task can be decomposed into four types of elements: a subgoal, a subtask, a resource, and %/or 
%a softgoal. Apart from those 
%Additionally to these two links, t
There are also the contribution links, which can vary from very positive to very  negative. %\ana{dizer que é para softgoals, similarmente ao que se fez para as outras duas relações??}
\ana{vale a pena deixar esta seção para esta comunidade? se sim, posso reduzir para ser max tamanho da section B, se acharem que vale a pena}

\subsection{Related studies}
\label{sec:related_studies}
 
This paper extends our\ana {a} previous work aimed at %where our goal was to evaluate 
evaluating the effect of the layout guidelines on the \textit{i*} novice stakeholders' ability to understand and review \textit{i*} models \cite{Santos2016RE}.\ana{remover esta ref ou dar a ref como se não fosse nossa, removendo "our"?? cleaned the rest}
A quasi-experiment was performed where participants were given two understanding and two reviewing tasks. Both tasks
involved a model with a bad layout and another model following the \textit{i*} layout guidelines. 
%We evaluated t
The impact of layouts was evaluated by combining the success level in those tasks and the required effort to accomplish them. 
Effort was assessed using time, perceived complexity (with NASA TLX), and eye-tracking data. The results revealed that the participants were more successful in understanding than in reviewing tasks. However, %we found 
no statistically significant difference was found in the success, time taken, or perceived complexity, between tasks conducted with models with a bad layout and models with a good layout. 

%\subsection{Relevance to practice}
%\label{sec:relevance_practice}
%Although well-known in the RE community (its main reference \cite{Yu1995} has been referenced over 1500 times, %according to Google Scholar), \textit{i*} is, as most other requirements languages, poorly understood by naïve %users \cite{Caire2013RE}. In this paper we are exploring the extent to which this problem can be mitigated by %using a more cognitive effective concrete syntax for \textit{i*}.
%%\ana{sugestão: levar isto para a introdução do paper. acho que serviria logo de início tb para motivação do %trabalho} 
%%\joao{acho que na intro fica melhor sim, isso não é bem background}
